FLIPS: Federated Learning using Intelligent Participant Selection

This paper presents the design and implementation of FLIPS, a middleware system to manage data and participant heterogeneity in federated learning (FL) training workloads. In particular, we examine the benefits of label distribution clustering on participant selection in federated learning. FLIPS clusters parties involved in an FL training job based on the label distribution of their data apriori, and during FL training, ensures that each cluster is equitably represented in the participants selected. FLIPS can support the most common FL algorithms, including FedAvg, FedProx, FedDyn, FedOpt and FedYogi. To manage platform heterogeneity and dynamic resource availability, FLIPS incorporates a straggler management mechanism to handle changing capacities in distributed, smart community applications. Privacy of label distributions, clustering and participant selection is ensured through a trusted execution environment (TEE). Our comprehensive empirical evaluation compares FLIPS with random participant selection, as well as three other "smart" selection mechanisms - Oort, TiFL and gradient clustering using two real-world datasets, two benchmark datasets, two different non-IID distributions and three common FL algorithms (FedYogi, FedProx and FedAvg). We demonstrate that FLIPS significantly improves convergence, achieving higher accuracy by 17 - 20 % with 20 - 60 % lower communication costs, and these benefits endure in the presence of straggler participants.

==> commentedouttext.tex <==
from abstract

\begin{comment}

In this paper, we examine the benefits of label distribution clustering approach where 
parties with similar label distributions are clustered together. Confidentiality of data is ensured by using Trusted Execution Environments (TEEs) on the parties' and aggregator's side, where the sharing of label distributions and cluster computations happens. Once clustered, we can now perform federated learning on clients across different clusters to generate a more robust global model for classification. This helps represent all labels while aggregation, as each local model brings knowledge corresponding to different labels. Results indicate that this model converges faster than other baselines, reducing communication overheads.


The convergence of this global model is highly dependent on the data skewness on the clients' side. In an IID setting (where data corresponding to all labels is uniformly present on all clients), convergence can be achieved. In a non-IID setting (where each client has data corresponding to different labels), convergence may or may not be achieved in a reasonable time due to inconsistent local models. To reduce the time required for convergence involving non-IID data distributions, we propose a 
\end{comment}
 


















%    \item Sort and Partition (each device has n number of classes)
%Another Dataset Partitioning technique we consider is Sort partition, where we control a parameter n, which determines how many labels should be present at each client. 
%    \item Realistic Partition (if we plan on including the ECG dataset)

\begin{comment}
\subsection{Secure Multiparty Computation}

Another technique to perform label distribution clustering without label distribution vectors is clustering on a matrix called the agreement matrix computed using secure multiparty computation.


Every client trains a local model on their local data in this method. These models are trained until local convergence is reached. Each client then creates a TEE loaded with its local dataset and the matchmaker code. An attestation server runs on each client to verify the TEE's hardware. Once verified a client can send its model via a secure TLS channel to the other client's TEE. The model exchange is depicted in Figure~\ref{fig:sys:design:distributed}. Each client shares its local model with the other N-1 clients in a similar fashion. Confidentiality of the models is ensured by sharing them on TEEs residing on the client's machines.

Once each client receives models from the other N-1 client, the matchmaker code performs inference on the models received on the client's local dataset. This inference metric is the per-label accuracy vector. Hence, in a setting with N clients, each client performs N inferences on their local datasets using the models received from other clients. These inference vectors are then shared with the centralized match-maker using an architecture similar to Figure~\ref{fig:sys:design:tee}. 


At the centralized matchmaker, a matrix called the agreement matrix is formed. This is collated by collecting inference vectors from each client. Each element in the matrix $A_{m,n}$ corresponds to a per-label accuracy vector computed on client $n's$ dataset on client $m's$ model. 

Clients with similar label distributions will depict high accuracy on the labels present in their local datasets. Hence, clustering the inference vectors in the agreement matrix will give us clients with similar label distribution. 

\rbnote{Vinod's Idea}
Suppose there are N clients ${c_1, c_2, ...,c_N}$ each with dataset ${d_1, d_2, ..., d_N}$. Let $A_i$ be the per-label accuracy vector at client $c_i$ with dataset $d_i$.

Let $A_{i,j}$ be the per label accuracy vector with model from client $i$ and dataset from client $j$. Then let $S_k$ be every possible subset of $A_{i,j}$ of size $k$. 
For eg $S_2 = {{a_{1,2}, a_{2,3}}, {a_{4,5}, a_{7,8}}}$

We want to find the set of clients such that:

$max_{S_{k}} \mod{merge(A_{s})}$, where

\begin{itemize}
    \item $A_{s} = {a_{i,j}}, a_{i,j} \epsilon S_{k}$
    \item $merge()$ is the element-wise max of a set of vectors
    \item $\mod$ is the L-1 norm of a vector


\rbnote{We need to prove that clustering is an approximate solution for this. This will require TBD steps if we have n clients }


\end{itemize}




\subsubsection{Clustering the agreement matrix}

Once the agreement matrix is collated, we perform clustering to identify clients with similar label distribution. We employ a novel approach to perform this clustering.

We traverse the agreement matrix column-wise; this gives us inference vectors corresponding to model $i$ inferred on local datasets corresponding to clients $1,2,.....n$. Here, the trained model remains the same while the datasets differ at each inference vector. We perform OPTICS CLustering on this set of inference vectors. This is done for each model $M_{k}, where k \epsilon {1, n}$. This gives us cluster groups corresponding to n different models.

Next, we make an adjacency matrix where each element $K_{i,j}$ is the number of times inference vectors of clients $i,j$ were in the same cluster across different models. This matrix is symmetric across the diagonal. We then perform spectral clustering over this adjacency matrix. \rbnote{To add why we choose these methods}. This gives us clusters where clients with similar data/label distribution are clustered together. 

\subsubsection{Advantages of this method}

\begin{figure*}[t!]
\centering
\includegraphics[width=1\textwidth]{Figures/distributed_tee.pdf}
  \caption{Secure Multiparty Computation}
    \label{fig:sys:design:distributed}
\end{figure*}
\end{comment}


==> comparisonStrategy.tex <==


\nvnote{add stuff about optimizers}

==> dirichlet_allocation.tex <==
\nvnote{add this to section 4.2}

To partition a dataset across several parties, we use Dirichlet Allocation~\cite{https://doi.org/10.48550/arxiv.1905.12022} as in Tensorflow Federated~\cite{tff} and LEAF~\cite{caldas2018leaf}. 
In this, we sample $p \sim Dir_{N} (\alpha)$, where $\alpha$ is the 
control parameter and $p_{l,i}$ becomes the proportion of the number of 
data points of label $l$ allocated to the party $i$. Additionally, we ensure that the number of data points is the same for all parties. 
This is done to mitigate the effect of local epochs while 
training on the edge.   We experiment with 2 different values of $\alpha=0.3$ and $0.6$, popularly used~\cite{gao2022federated}. At each round, we sample 20 \% and 15 \% parties which is more than the number of clusters of similar parties formed in \ours.

\begin{comment}
When $\alpha \to 0$, each client only has 
data corresponding to one label, as shown in Figure~\ref{fig:dir:0}.    
When $\alpha \to \infty$, the label distribution is IID, and each 
client has data corresponding to all labels like in 
Figure~\ref{fig:dir:0}. \rbnote{We experiment with 4 different values 
of $\alpha$ which are $\to 0, 0.3, 0.6, \to \infty$ following~\cite{gao2022federated}, 
which can be seen in Figures~\ref{fig:dir:03},~\ref{fig:dir:06}.}



\begin{figure}[h]
\centering
\subfloat[$\alpha=0.3$ ]{{\includegraphics[width=0.22\textwidth]{Dirichlet_plots/dir_03_emnist.pdf}}%
    \label{fig:dir:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.22\textwidth] {Dirichlet_plots/dir_06_emnist.pdf}%
    \label{fig:dir:06}
    }%
  \quad
    \subfloat[$\alpha\to0$]{\includegraphics[width=0.22\textwidth] {Dirichlet_plots/dir_0_emnist.pdf}%
    \label{fig:dir:0}
    }%
  \quad
    \subfloat[$\alpha\to\infty$]{\includegraphics[width=0.22\textwidth] {Dirichlet_plots/dir_inf_emnist.pdf}%
    \label{fig:dir:inf}
    }%
  \caption{Label Distribution in Subsampled EMNIST dataset for 20 randomly chosen parties (out of 200) at different $\alpha$}
\end{figure}
\end{comment}


\begin{comment}
\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Dirichlet_plots/dir_03_emnist.pdf}
  \caption{Label Distribution in Subsampled EMNIST dataset for $\alpha=0.3$ for 20 randomly chosen parties}
    \label{fig:dir:ld03}
\end{figure}

\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Dirichlet_plots/dir_06_emnist.pdf}
  \caption{Label Distribution in Subsampled EMNIST dataset for $\alpha=0.6$ for 20 randomly chosen parties}
    \label{fig:dir:ld06}
\end{figure}


\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Dirichlet_plots/dir_0_emnist.pdf}
  \caption{Label Distribution in Subsampled EMNIST dataset for $\alpha\to0$ for 20 randomly chosen parties}
    \label{fig:dir:ld0}
\end{figure}


\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Dirichlet_plots/dir_inf_emnist.pdf}
  \caption{Label Distribution in Subsampled EMNIST dataset for $\alpha\to\infty$ for 20 randomly chosen parties}
    \label{fig:dir:ldinf}
\end{figure}
\end{comment}

==> discussion.tex <==
\section{Discussion}



%Does centralized clustering shrink the potential areas where this technique can be applied?
%What if there is no centralized aggregator?

==> ecg_plots.tex <==
\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedavg_03.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.3$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:ecg03:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedavg_06.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.6$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:ecg06:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedprox_03.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.3$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:ecg03:fedprox}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedprox_06.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.6$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:ecg06:fedprox}
\end{figure}
\end{comment}







\begin{comment}
\begin{figure}[h]
\centering
\subfloat[$\alpha=0.3$]{{\includegraphics[width=0.4\textwidth]{Plots/mit_10_20_strg_ecg_yogi_03.pdf}}%
    \label{fig:mit:strg:03}
    }% 
    \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.4\textwidth] {Plots/mit_10_20_strg_ecg_yogi_06.pdf}%
    \label{fig:mit:strg:06}
    }%
  
  \caption{Convergence plots on MIT BIH ECG Dataset in the presence of Stragglers}
  \label{fig:mit:strg:all}
\end{figure}

    \begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$]{{\includegraphics[width=0.4\textwidth]{Plots/mit_20_strg_ecg_yogi_03.pdf}}%
    \label{fig:mit:20:strg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.4\textwidth] {Plots/mit_20_strg_ecg_yogi_06.pdf}%
    \label{fig:mit:20:strg:06}
    }%
  
  \caption{Convergence plots on MIT BIH ECG Dataset in the presence of 20 \% Stragglers}
  \label{fig:mit:20strg:all}
\end{figure*}
\end{comment}


==> fashion_mnist_plots.tex <==
\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/fashion_mnist_fedavg_03.pdf}
  \caption{Convergence plots on Fashion MNIST dataset with $\alpha = 0.3$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:fashion_mnist03:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/fashion_mnist_fedavg_06.pdf}
  \caption{Convergence plots on Fashion MNIST dataset with $\alpha = 0.6$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:fashion_mnist06:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/fashion_mnist_fedprox_03.pdf}
  \caption{Convergence plots on Fashion MNIST dataset with $\alpha = 0.3$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:fashion_mnist03:fedprox}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/fashion_mnist_fedprox_06.pdf}
  \caption{Convergence plots on Fashion MNIST dataset with $\alpha = 0.6$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:fashion_mnist06:fedprox}
\end{figure}

\end{comment}

\begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$ with \textit{FedAvg}]{{\includegraphics[width=0.4\textwidth]{Plots/fashion_mnist_fedavg_03.pdf}}%
    \label{fig:fashionmnist:fedavg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$ with \textit{FedAvg}]{\includegraphics[width=0.4\textwidth] {Plots/fashion_mnist_fedavg_06.pdf}%
    \label{fig:fashionmnist:fedavg:06}
    }%
  \quad
    \subfloat[$\alpha=0.3$ with \textit{FedProx}]{\includegraphics[width=0.4\textwidth] {Plots/fashion_mnist_fedprox_03.pdf}%
    \label{fig:fashionmnist:fedprox:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$ with \textit{FedProx}]{\includegraphics[width=0.4\textwidth] {Plots/fashion_mnist_fedprox_06.pdf}%
    \label{fig:fashionmnist:fedprox:06}
    }%
  \caption{Convergence plots on the Fashion MNIST dataset. The results depict the benefit of using FLIPS along with \textit{FedAvg} and \textit{FedProx}}
  \label{fig:fashionmnist:all}
\end{figure*}

==> femnist_plots.tex <==
\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/femnist_fedavg_03.pdf}
  \caption{Convergence plots on FEMNIST dataset with $\alpha = 0.3$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:femnist03:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/femnist_fedavg_06.pdf}
  \caption{Convergence plots on FEMNIST dataset with $\alpha = 0.6$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:femnist06:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/femnist_fedprox_03.pdf}
  \caption{Convergence plots on FEMNIST dataset with $\alpha = 0.3$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:femnist03:fedprox}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/femnist_fedprox_06.pdf}
  \caption{Convergence plots on FEMNIST dataset with $\alpha = 0.6$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:femnist06:fedprox}
\end{figure}




\begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$ with \textit{FedAvg}]{{\includegraphics[width=0.4\textwidth]{Plots/femnist_fedavg_03.pdf}}%
    \label{fig:femnist:fedavg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$ with \textit{FedAvg}]{\includegraphics[width=0.4\textwidth] {Plots/femnist_fedavg_06.pdf}%
    \label{fig:femnist:fedavg:06}
    }%
  \quad
    \subfloat[$\alpha=0.3$ with \textit{FedProx}]{\includegraphics[width=0.4\textwidth] {Plots/femnist_fedprox_03.pdf}%
    \label{fig:femnist:fedprox:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$ with \textit{FedProx}]{\includegraphics[width=0.4\textwidth] {Plots/femnist_fedprox_06.pdf}%
    \label{fig:femnist:fedprox:06}
    }%
  \caption{Convergence plots on the subsampled FEMNIST dataset. The results depict the benefit of using FLIPS along with \textit{FedAvg} and \textit{FedProx}}
    \label{fig:femnist:all}
\end{figure*}

\end{comment}






\begin{comment}

\begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$ in the presence of stragglers]{{\includegraphics[width=0.9\columnwidth]{Plots/femnist_10_20_strg_ecg_yogi_03.pdf}}%
    \label{fig:femnist:strg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$ in the presence of stragglers]{\includegraphics[width=0.9\columnwidth] {Plots/femnist_10_20_strg_ecg_yogi_06.pdf}%
    \label{fig:femnist:strg:06}
    }%
  
  \caption{Convergence plots on FEMNIST dataset in the presence of Stragglers}
  \label{fig:femnist:strg:all}
\end{figure*}



    \begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$]{{\includegraphics[width=0.4\textwidth]{Plots/femnist_20_strg__yogi_03.pdf}}%
    \label{fig:femnist:20:strg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.4\textwidth] {Plots/femnist_20_strg__yogi_03.pdf}%
    \label{fig:femnist:20:strg:06}
    }%
  
  \caption{Convergence plots on FEMNIST dataset in the presence of 10 \% Stragglers}
  \label{fig:femnist:20strg:all}
\end{figure*}


\end{comment}



==> related.tex <==

\section{Related Work}

Make sure to add all the papers you read here. we can filter later.




https://proceedings.mlr.press/v151/jee-cho22a/jee-cho22a.pdf = PMLR Gauri Joshi 






Mohak Chaddha our main competitor?
FedLesScan: Mitigating Stragglers in Serverless Federated Learning
Elzohairy, Mohamed, Chadha, Mohak, Jindal, Anshul, Grafberger, Andreas, Gu, Jianfeng, Gerndt, Michael, and Abboud, Osama
In 2022 IEEE 10th International Conference on Big Data (IEEE BigData) 2022 
https://www.youtube.com/watch?v=p4JkJFKqWRg&feature=youtu.be










@inproceedings{
gao2022federated,
title={FedDC: Federated Learning with Non-IID Data via Local Drift Decoupling and Correction},
author={Liang Gao and Huazhu Fu and Li Li and Yingwen Chen and Ming Xu and Cheng-Zhong Xu},
booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
year={2022}
}


Karimireddy, S.P., Kale, S., Mohri, M., Reddi, S., Stich, S. &amp; Suresh, A.T.. (2020). SCAFFOLD: Stochastic Controlled Averaging for Federated Learning. <i>Proceedings of the 37th International Conference on Machine Learning</i>, in <i>Proceedings of Machine Learning Research</i> 119:5132-5143 Available from https://proceedings.mlr.press/v119/karimireddy20a.html.

@article{ZHU2021371,
title = {Federated learning on non-IID data: A survey},
journal = {Neurocomputing},
volume = {465},
pages = {371-390},
year = {2021},
issn = {0925-2312},
doi = {https://doi.org/10.1016/j.neucom.2021.07.098},
url = {https://www.sciencedirect.com/science/article/pii/S0925231221013254},
author = {Hangyu Zhu and Jinjin Xu and Shiqing Liu and Yaochu Jin},
keywords = {Federated learning, Machine learning, Non-IID data, Privacy preservation},
abstract = {Federated learning is an emerging distributed machine learning framework for privacy preservation. However, models trained in federated learning usually have worse performance than those trained in the standard centralized learning mode, especially when the training data are not independent and identically distributed (Non-IID) on the local devices. In this survey, we provide a detailed analysis of the influence of Non-IID data on both parametric and non-parametric machine learning models in both horizontal and vertical federated learning. In addition, current research work on handling challenges of Non-IID data in federated learning are reviewed, and both advantages and disadvantages of these approaches are discussed. Finally, we suggest several future research directions before concluding the paper.}
}

==> reviews.tex <==
\section{Reviews from ICDCS 2023}

\rbnote{REVIEW 1}
SCORE: 1 (weak accept)


The paper addresses the problem of participant selection in Federated Learning (FL) to improve model convergence. The authors highlight that current approaches are suboptimal and propose a method that leverages clustering techniques based on label distributions. They also introduce a private mechanism using trusted execution environments (TEEs) to securely cluster participants in FL jobs based on their data's label distributions. The authors provide empirical evaluations using three real-world datasets, demonstrating better convergence and reduced communication overheads with their approach.

To better emphasize the advantages and trade-offs of the proposed method, consider offering a more detailed comparison with other participant selection approaches, 




focusing on aspects such as model convergence, computational efficiency, and communication overheads.
\rbnote{Add system metrics ? Model convergence is incorporated in the graphs. }



Please also do clarify the importance of label distribution for participant selection in FL and provide more context on key concepts like non-IID data for readers who may be less familiar with FL.
We did, highlighting the non-IID issue.

Lastly, it would be good to enhance the paper with a more comprehensive literature review, citing recent and relevant works in the field of participant selection in FL. This will help contextualize the proposed method within the broader research landscape.


\rbnote{REVIEW 2} SCORE: -1 (weak reject)

This paper presents a federated learning that do not randomly select participants. The key idea is to cluster participants based on labels and select a party from each cluster in a round robin manner. The work is evaluated with three datasets and a real world scenario, and compared against random selection.

The idea of selecting participants based on label distribution seems beneficial. However, it requires the system to have global information about the data and distribution among the participants, which is not realistic. 

The benefits of reduced communication come from the reduced number of participants. The accuracy relies on the quality of clustering. The paper doesn't discuss situations such as what if clustering is not good quality, what if the number of participants are not selected well, etc. 

\rbnote{Compare more techniques (Oort, IFCA) if python implementation is available.
Oort Possible
IFCA looks possible
Clustering models is also used to find similar clients}

\textbf{The work is only compared to random selection.
}


\rbnote{REVIEW 3} SCORE: -1 (weak reject)
The paper aims to develop methods for smartly selecting participants for a federate learning task.
The basic question is well motivated but the contribution of the paper are not clear. The basic idea is to cluster the participants and then select a subset from these clusters. The basic ideas used in the paper seemed very straightforward.




\rbnote{
\begin{itemize}
    \item Distributed Clustering*
\item Proof Carrying Code
\item Proving that label distribution mentioned by the parties is correct.
\item How to measure the diversity of the models*
\item Measure of diversity : per label accuracy . Metric for diversity (VLDB)
\item Get a diverse model fast
\item Convergence and Communication part
\item Parties drop off : still get a more diverse model.
\item Compare against more techniques* (Random + Oort + IFCA + model clustering…)
 \item Organize the results of the experiments
\end{itemize}
}





\rbnote{IDEAS:
\begin{itemize}
    \item Add math - mathematical formulation of finding similar clients.
    \item Systemic utility via the effect of stragglers.
    \item If we find the average straggler rate to be $x\%$, we choose $x\%$ more parties in FL.
    \item This extra $x\%$ could be defined by exploiting used clients from previous iterations.
\end{itemize}
}



\rbnote{To ask Jayaram: 1) basic comparison experiments with all optimizers on 1 dataset or }

==> sk_ham_plots.tex <==
\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedavg_03.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.3$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:ecg03:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedavg_06.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.6$ and \textit{FedAvg} algorithm. The results depict the benefit of using FLIPS along with \textit{FedAvg}}
    \label{fig:plot:ecg06:fedavg}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedprox_03.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.3$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:ecg03:fedprox}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{Plots/mit_ecg_fedprox_06.pdf}
  \caption{Convergence plots on MIT-BIH ECG dataset with $\alpha = 0.6$ and \textit{FedProx} algorithm. The results depict the benefit of using FLIPS along with \textit{FedProx}}
    \label{fig:plot:ecg06:fedprox}
\end{figure}
\end{comment}








\begin{comment}

\begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$]{{\includegraphics[width=0.4\textwidth]{Plots/sk_10_20_strg_ecg_yogi_03.pdf}}%
    \label{fig:sk:strg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.4\textwidth] {Plots/sk_10_20_strg_ecg_yogi_06.pdf}%
    \label{fig:sk:strg:06}
    }%
  
  \caption{Convergence plots on HAM10000 (Skin Lesions) Dataset in the presence of Stragglers}
  \label{fig:sk:strg:all}
\end{figure*}
    \begin{figure*}[h]
\centering
\subfloat[$\alpha=0.3$]{{\includegraphics[width=0.4\textwidth]{Plots/sk_20_strg__yogi_03.pdf}}%
    \label{fig:sk:20:strg:03}
    }%
  \quad
    \subfloat[$\alpha=0.6$]{\includegraphics[width=0.4\textwidth] {Plots/sk_20_strg__yogi_06.pdf}%
    \label{fig:sk:20:strg:06}
    }%
  
  \caption{Convergence plots on HAM10000 (Skin Lesions) Dataset in the presence of 20 \% Stragglers}
  \label{fig:sk:20strg:all}
\end{figure*}
\end{comment}


==> tables_results.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{FEMNIST dataset : Rounds required to attain Target Accuracy (80\%)}

\begin{tabular}{cc|cccccccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Setting}}} & \multicolumn{8}{c}{\textbf{Rounds required to attain 80 \% accuracy, FL Algorithm : FedYoGi}}                                                                                                     \\ \cline{3-10} 
\multicolumn{2}{c|}{}                                  & \multicolumn{4}{c|}{\textbf{0 \% Stragglers}}                                            & \multicolumn{2}{c|}{\textbf{10 \% Stragglers}}      & \multicolumn{2}{c}{\textbf{20 \% Stragglers}} \\ \hline
\textbf{alpha}        & \textbf{participant \%}        & \textbf{Random} & \textbf{FLIPS} & \textbf{OORT} & \multicolumn{1}{c|}{\textbf{GradCls}} & \textbf{FLIPS} & \multicolumn{1}{c|}{\textbf{OORT}} & \textbf{FLIPS}         & \textbf{OORT}        \\ \hline
0.3                   & 20                             & 146             & 62             & 81            & \multicolumn{1}{c|}{168}              & 69             & \multicolumn{1}{c|}{102}           & 78                     & 85                   \\
0.3                   & 15                             & 181             & 62             & 83            & \multicolumn{1}{c|}{168}                 & 76             & \multicolumn{1}{c|}{105}           & 79                     & 103                  \\
0.6                   & 20                             & 107             & 68             & 66            & \multicolumn{1}{c|}{89}                 & 89             & \multicolumn{1}{c|}{69}            & 89                     & 84                   \\
0.6                   & 15                             & 115             & 75             & 55            & \multicolumn{1}{c|}{115}                 & 86             & \multicolumn{1}{c|}{83}            & 78                     & 88                  
\end{tabular}
\label{femnist:rounds}
\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{FEMNIST dataset: highest accuracy attained within the rounds threshold}
\begin{tabular}{cc|cccccccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Setting}}} & \multicolumn{8}{c}{\textbf{Highest accuracy attained, FL Algorithm : FedYoGi}}                                                                                                                    \\ \cline{3-10} 
\multicolumn{2}{c|}{}                                  & \multicolumn{4}{c|}{\textbf{0 \% Stragglers}}                                            & \multicolumn{2}{c|}{\textbf{10 \% Stragglers}}      & \multicolumn{2}{c}{\textbf{20 \% Stragglers}} \\ \hline
\textbf{alpha}        & \textbf{participant \%}        & \textbf{Random} & \textbf{FLIPS} & \textbf{OORT} & \multicolumn{1}{c|}{\textbf{GradCls}} & \textbf{FLIPS} & \multicolumn{1}{c|}{\textbf{OORT}} & \textbf{FLIPS}         & \textbf{OORT}        \\ \hline
0.3                   & 20                             & 80.97           & 86.60          & 85.27         & \multicolumn{1}{c|}{80.97}            & 86.75          & \multicolumn{1}{c|}{83.21}         & 85.85                  & 84.69                \\
0.3                   & 15                             & 82.60           & 86.86          & 84.61         & \multicolumn{1}{c|}{82.51}            & 86.68          & \multicolumn{1}{c|}{85.24}         & 86.78                  & 84.74                \\
0.6                   & 20                             & 83.94           & 85.37          & 85.36         & \multicolumn{1}{c|}{84.21}            & 85.13          & \multicolumn{1}{c|}{85.44}         & 85.69                  & 85.00                \\
0.6                   & 15                             & 82.44           & 84.51          & 85.51         & \multicolumn{1}{c|}{83.08}            & 85.00          & \multicolumn{1}{c|}{86.19}         & 86.04                  & 84.87               
\end{tabular}
\label{femnist:accuracy}

\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{FEMNIST Dataset: Rounds required to attain Target Accuracy (80\%)}

\begin{tabular}{cc|cccccccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Setting}}} & \multicolumn{8}{c}{\textbf{Rounds required to attain 80 \% accuracy, FL Algorithm : FedProx}}                                                                                                  \\ \cline{3-10} 
\multicolumn{2}{c|}{}                                  & \multicolumn{4}{c|}{\textbf{0 \% Stragglers}}                                            & \multicolumn{2}{c|}{\textbf{10 \% Stragglers}}      & \multicolumn{2}{c}{\textbf{20 \% Stragglers}} \\ \hline
\textbf{alpha}        & \textbf{participant \%}        & \textbf{Random} & \textbf{FLIPS} & \textbf{OORT} & \multicolumn{1}{c|}{\textbf{GradCls}} & \textbf{FLIPS} & \multicolumn{1}{c|}{\textbf{OORT}} & \textbf{FLIPS}         & \textbf{OORT}        \\ \hline
0.3                   & 20                             & 128             & 47             & 71            & \multicolumn{1}{c|}{157}              & 65             & \multicolumn{1}{c|}{130}           & 78                     & 128                  \\
0.3                   & 15                             & 104             & 54             & 70            & \multicolumn{1}{c|}{149}              & 72             & \multicolumn{1}{c|}{118}           & 67                     & 156                  \\
0.6                   & 20                             & 84              & 62             & 53            & \multicolumn{1}{c|}{84}               & 90             & \multicolumn{1}{c|}{82}            & 80                     & 77                   \\
0.6                   & 15                             & 86              & 56             & 62            & \multicolumn{1}{c|}{88}               & 78             & \multicolumn{1}{c|}{91}            & 86                     & 85                  
\end{tabular}
\label{femnist:rounds:prox}

\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{FEMNIST Dataset: : highest accuracy attained within the rounds threshold}

\begin{tabular}{cc|cccccccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Setting}}} & \multicolumn{8}{c}{\textbf{Highest Accuracy attained, FL Algorithm : FedProx}}                                                                                                                 \\ \cline{3-10} 
\multicolumn{2}{c|}{}                                  & \multicolumn{4}{c|}{\textbf{0 \% Stragglers}}                                            & \multicolumn{2}{c|}{\textbf{10 \% Stragglers}}      & \multicolumn{2}{c}{\textbf{20 \% Stragglers}} \\ \hline
\textbf{alpha}        & \textbf{participant \%}        & \textbf{Random} & \textbf{FLIPS} & \textbf{OORT} & \multicolumn{1}{c|}{\textbf{GradCls}} & \textbf{FLIPS} & \multicolumn{1}{c|}{\textbf{OORT}} & \textbf{FLIPS}         & \textbf{OORT}        \\ \hline
0.3                   & 20                             & 82.80           & 90.43          & 86.59         & \multicolumn{1}{c|}{81.78}            & 87.33          & \multicolumn{1}{c|}{83.21}         & 86.56                  & 83.81                \\
0.3                   & 15                             & 83.24           & 89.72          & 86.51         & \multicolumn{1}{c|}{83.34}            & 87.02          & \multicolumn{1}{c|}{83.81}         & 86.82                  & 82.43                \\
0.6                   & 20                             & 85.60           & 88.99          & 87.45         & \multicolumn{1}{c|}{85.05}            & 85.23          & \multicolumn{1}{c|}{86.11}         & 85.72                  & 85.91                \\
0.6                   & 15                             & 85.58           & 89.27          & 86.49         & \multicolumn{1}{c|}{83.91}            & 86.20          & \multicolumn{1}{c|}{85.28}         & 85.13                  & 85.35               
\end{tabular}
\label{femnist:accuracy:prox}

\end{table*}














\begin{comment}
\begin{figure} [h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/vgg16_rvl.png}
        \caption{Training VGG16 on RVL CDIP dataset. Here each client has 2 labels present}

    \label{fig:vgg16:rvl:1}
\end{figure}
\end{comment}
\begin{comment}
\begin{table}[]
\centering
\caption{Number of rounds required to attain target accuracy for FashionMNIST trained on Le-Net-5}
\begin{tabular}{lll|ll}
\hline
\multicolumn{3}{l|}{\textbf{Setting}}             & \multicolumn{2}{l}{\textbf{Rounds}}      \\ \hline
\textbf{Participation \%} & \textbf{Dir} & \textbf{Target Acc} & \textbf{FedProx}  & \textbf{FLIPS} \\ \hline
10           & 0.6          & 80                  & 109               & 19                   \\ \hline
5            & 0.6          & 80                  & \textgreater{}200 & 74                   \\ \hline
2            & 0.6          & 80                  & \textgreater{}200 & 57                   \\ \hline
10           & 0.3          & 80                  & \textgreater{}200 & 64                   \\ \hline
5            & 0.3          & 80                  & 106               & 78                   \\ \hline
2            & 0.3          & 80                  & \textgreater{}200 & 18                   \\ \hline
\end{tabular}
\label{table:rounds:fedmnist}
\end{table}


\begin{table*}[]
\centering
\caption{Number of communication rounds required to attain 80\% target accuracy for FashionMNIST trained on Le-Net-5. The No. of communication rounds reduced and bandwidth saved is a result of using \ours}
\begin{tabular}{cc|cccc|cc|cc}
\hline
\multicolumn{2}{c|}{\textbf{Setting}}    & \multicolumn{4}{c|}{\textbf{Communication Rounds Required}}                                                                                                                  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Communication\\ Rounds Reduction\end{tabular}}}                               & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Bandwidth \\ Saved (\%)\end{tabular}}}                                     \\ \hline
\textbf{Dir-alpha} & \textbf{\% Parties} & \textbf{FedAvg}   & \textbf{FedProx}  & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} \\ \hline
0.6                & 20                  & 69                & 67                & 67                                                               & 63                                                                & 2                                                                & 4                                                                 & 2.90                                                             & 5.97                                                              \\
0.6                & 15                  & 178               & 71                & 65                                                               & 57                                                                & 113                                                              & 14                                                                & 63.48                                                            & 19.72                                                             \\
0.6                & 10                  & 56                & 109               & 50                                                               & 65                                                                & 6                                                                & 44                                                                & 10.71                                                            & 40.37                                                             \\
0.6                & 5                   & 32                & \textgreater{}200 & 32                                                               & 69                                                                & 0                                                                & 131                                                               & 0.00                                                             & 65.50                                                             \\
0.3                & 20                  & 47                & 71                & 47                                                               & 71                                                                & 0                                                                & 0                                                                 & 0.00                                                             & 0.00                                                              \\
0.3                & 15                  & 99                & 156               & 79                                                               & 86                                                                & 20                                                               & 70                                                                & 20.20                                                            & 44.87                                                             \\
0.3                & 10                  & 80                & \textgreater{}200 & 63                                                               & 81                                                                & 17                                                               & 119                                                               & 21.25                                                            & 59.50                                                             \\
0.3                & 5                   & \textgreater{}200 & 106               & 86                                                               & 85                                                                & 114                                                              & 21                                                                & 57.00                                                            & 19.81                                                             \\ \hline
\end{tabular}

\label{table:rounds:fashionmnist}

\end{table*}


\begin{comment}
\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Figures/fashion_mnist.pdf}
  \caption{Number of rounds required to attain 80\% target accuracy for FashionMNIST trained on Le-Net-5}
    \label{fig:res:fashion:mnist}
\end{figure}



\begin{figure}[]
\centering
\includegraphics[width=0.45\textwidth]{Figures/ecg_results.pdf}
  \caption{Number of rounds required to attain $50 \%$ target accuracy (this is the average of per label accuracy, as the number of samples for each label in the dataset are not equal) for MIT-BIH Arrhythmia Dataset trained on 1D CNN}
    \label{fig:res:mit:dataset}
\end{figure}


\begin{table*}[]
\centering
\caption{Number of rounds required to attain $50 \%$ target accuracy for MIT-BIH Arrhythmia Dataset trained on 1D CNN. The No. of communication rounds reduced and bandwidth saved is a result of using \ours}
\begin{tabular}{cc|cccc|cc|cc}
\hline
\multicolumn{2}{c|}{\textbf{Setting}}    & \multicolumn{4}{c|}{\textbf{Communication Rounds Required}}                                                                                                                  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Communication\\ Rounds Reduction\end{tabular}}}                               & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Bandwidth \\ Saved (\%)\end{tabular}}}                                     \\ \hline
\textbf{Dir-alpha} & \textbf{\% Parties} & \textbf{FedAvg}   & \textbf{FedProx}  & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} \\ \hline
0.6                & 20                  & \textgreater{}200 & \textgreater{}200 & 87                                                               & 134                                                               & 113                                                              & 66                                                                & 56.50                                                            & 33.00                                                             \\
0.6                & 15                  & \textgreater{}200 & \textgreater{}200 & 135                                                              & 173                                                               & 65                                                               & 27                                                                & 32.50                                                            & 13.50                                                             \\
0.6                & 10                  & \textgreater{}200 & \textgreater{}200 & 150                                                              & 178                                                               & 50                                                               & 22                                                                & 25.00                                                            & 11.00                                                             \\
0.6                & 5                   & \textgreater{}200 & \textgreater{}200 & 127                                                              & 43                                                                & 73                                                               & 157                                                               & 36.50                                                            & 78.50                                                             \\
0.3                & 20                  & \textgreater{}200 & \textgreater{}200 & 64                                                               & 52                                                                & 136                                                              & 148                                                               & 68.00                                                            & 74.00                                                             \\
0.3                & 15                  & \textgreater{}200 & \textgreater{}200 & 55                                                               & 72                                                                & 145                                                              & 128                                                               & 72.50                                                            & 64.00                                                             \\
0.3                & 10                  & \textgreater{}200 & \textgreater{}200 & 45                                                               & 41                                                                & 155                                                              & 159                                                               & 77.50                                                            & 79.50                                                             \\
0.3                & 5                   & \textgreater{}200 & \textgreater{}200 & 45                                                               & 45                                                                & 155                                                              & 155                                                               & 77.50                                                            & 77.50                                                             \\ \hline
\end{tabular}

\label{table:rounds:ecg:arrythmia}

\end{table*}



\begin{table*}[]
\centering
\caption{Number of rounds required to attain $85 \%$ target accuracy for Subsampled - EMNIST dataset trained on Le-Net-5. The No. of communication rounds reduced and bandwidth saved is a result of using \ours}
\begin{tabular}{cc|cccc|cc|cc}
\hline
\multicolumn{2}{c|}{\textbf{Setting}}    & \multicolumn{4}{c|}{\textbf{Communication Rounds Required}}                                                                                                                  & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Communication\\ Rounds Reduction\end{tabular}}}                               & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Bandwidth \\ Saved (\%)\end{tabular}}}                                     \\ \hline
\textbf{Dir-alpha} & \textbf{\% Parties} & \textbf{FedAvg}   & \textbf{FedProx}  & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} \\ \hline
0.6                & 20                  & 197               & 167               & 142                                                              & 156                                                               & 55                                                               & 11                                                                & 27.92                                                            & 6.59                                                              \\
0.6                & 15                  & 156               & 159               & 146                                                              & 134                                                               & 10                                                               & 25                                                                & 6.41                                                             & 15.72                                                             \\
0.6                & 10                  & 150               & 158               & 137                                                              & 137                                                               & 13                                                               & 21                                                                & 8.67                                                             & 13.29                                                             \\
0.6                & 5                   & 151               & 170               & 134                                                              & 149                                                               & 17                                                               & 51                                                                & 11.26                                                            & 12.35                                                             \\
0.3                & 20                  & \textgreater{}200 & \textgreater{}200 & 120                                                              & 110                                                               & 80                                                               & 90                                                                & 40.00                                                            & 45.00                                                             \\
0.3                & 15                  & \textgreater{}200 & \textgreater{}200 & 128                                                              & 141                                                               & 72                                                               & 59                                                                & 36.00                                                            & 29.50                                                             \\
0.3                & 10                  & \textgreater{}200 & \textgreater{}200 & 124                                                              & 132                                                               & 76                                                               & 68                                                                & 38.00                                                            & 34.00                                                             \\
0.3                & 5                   & \textgreater{}200 & 169               & 139                                                              & 139                                                               & 61                                                               & 30                                                                & 30.50                                                            & 17.75                                                             \\ \hline
\end{tabular}

\label{table:rounds:emnist}

\end{table*}

\begin{comment}
\begin{table}[]
\begin{tabular}{cc|cccc|ll|}
\hline
\multicolumn{2}{c|}{\textbf{Setting}}    & \multicolumn{4}{c|}{\textbf{Rounds}}                                                                                                                                         & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Bandwidth \\ Saved\end{tabular}}}                                                                                      \\ \hline
\textbf{Dir-alpha} & \textbf{\% Parties} & \textbf{FedAvg}   & \textbf{FedProx}  & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedAvg\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FLIPS \\ FedProx\end{tabular}}} \\ \hline
0.6                & 20                  & 197               & 167               & 142                                                              & 156                                                               &                                                                                      &                                                                                        \\
0.6                & 15                  & 156               & 159               & 146                                                              & 134                                                               &                                                                                      &                                                                                        \\
0.6                & 10                  & 150               & 158               & 137                                                              & 137                                                               &                                                                                      &                                                                                        \\
0.6                & 5                   & 151               & 170               & 134                                                              & 149                                                               &                                                                                      &                                                                                        \\
0.3                & 20                  & \textgreater{}200 & \textgreater{}200 & 120                                                              & 110                                                               &                                                                                      &                                                                                        \\
0.3                & 15                  & \textgreater{}200 & \textgreater{}200 & 128                                                              & 141                                                               &                                                                                      &                                                                                        \\
0.3                & 10                  & \textgreater{}200 & \textgreater{}200 & 124                                                              & 132                                                               &                                                                                      &                                                                                        \\
0.3                & 5                   & \textgreater{}200 & 169               & 139                                                              & 139                                                               &                                                                                      &                                                                                        \\ \hline
\end{tabular}
\end{table}

\end{comment}
